ENWAR: A RAG-empowered Multi-Modal LLM Framework for Wireless Environment Perception

Large language models (LLMs) hold significant promise in advancing network management and orchestration in 6G and beyond networks. However, existing LLMs are limited in domain-specific knowledge and their ability to handle multi-modal sensory data, which is critical for real-time situational awareness in dynamic wireless environments. This paper addresses this gap by introducing ENWAR, an ENvironment-aWARe retrieval augmented generation-empowered multi-modal LLM framework. ENWAR seamlessly integrates multi-modal sensory inputs to perceive, interpret, and cognitively process complex wireless environments to provide human-interpretable situational awareness. ENWAR is evaluated on the GPS, LiDAR, and camera modality combinations of DeepSense6G dataset with state-of-the-art LLMs such as Mistral-7b/8x7b and LLaMa3.1-8/70/405b. Compared to general and often superficial environmental descriptions of these vanilla LLMs, ENWAR delivers richer spatial analysis, accurately identifies positions, analyzes obstacles, and assesses line-of-sight between vehicles. Results show that ENWAR achieves key performance indicators of up to 70% relevancy, 55% context recall, 80% correctness, and 86% faithfulness, demonstrating its efficacy in multi-modal perception and interpretation.

==> acronym.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother


\acrodef{LLM}[LLM]{large language model}
%\acrodef{LMM}[LMM]{large multi-modal model}
\acrodef{MLLM}[MLLM]{multi-modal large language model}
\acrodef{RAG}[RAG]{retrieval-augmented generation}
\acrodef{ISAC}[ISAC]{integrated sensing and communication}
\acrodef{ZSM}[ZSM]{zero-touch network and service management}
\acrodef{DT}[DT]{digital twin}
\acrodef{I2T}[I2T]{image-to-text}
\acrodef{GTE}[GTE]{General Text Embeddings}
\acrodef{GLUE}[GLUE]{General Language Understanding Evaluation}
\acrodef{MMLU}[MMLU]{Massive Multitask Language Understanding}

%% Predefined Acronyms %%%

\acrodef{IoT}[IoT]{Internet of things}
\acrodef{PDCP}[PDCP]{packet data convergence protocol}
\acrodef{RATs}[RATs]{radio access technologies}
% \acrodefplural{RAT}[RAT]{radio access technologies}
\acrodef{AP}[AP]{access point}
\acrodef{BS}[BS]{base station}
\acrodef{MP-TCP}[MP-TCP]{Multipath transmission control protocol}
\acrodef{5QI}[5QI]{\ac{5G} \ac{QoS} identifier}
\acrodef{NSI}[NSI]{network slice instance}
\acrodef{ATSSS}[ATSSS]{access traffic steering, switching and splitting}
\acrodef{CA}[CA]{coordination area}
\acrodef{TRP}[TRP]{transmission-reception point}
\acrodef{SON}[SON]{self-organizing network}
\acrodef{V2X}[V2X]{vehicle-to-everything}
\acrodef{eMBB}[eMBB]{enhanced mobile broadband}
\acrodef{mMTC}[mMTC]{massive machine type communication}
\acrodef{uRLLC}[uRLLC]{ultra-reliable low latency communication}
\acrodef{CoMP}[CoMP]{coordinated multipoint}
\acrodef{LTE}[LTE]{Long Term Evolution}
\acrodef{LTE-A}[LTE-A]{LTE-Advanced}
\acrodef{3GPP}[3GPP]{3rd Generation Partnership Project}
\acrodef{FFR}[FFR]{fractional frequency reuse}
\acrodef{SFR}[SFR]{soft frequency reuse}
\acrodef{ICI}[ICI]{inter-cell interference}
\acrodef{ICIC}[ICIC]{inter-cell interference coordination}
\acrodef{eICIC}[eICIC]{enhanced \ac{ICIC}}
\acrodef{ABS}[ABS]{absolute blank subframe}
\acrodef{TP}[TP]{transmission point}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{eNB}[eNB]{eNodeB}
\acrodef{RAN}[RAN]{radio access network}
\acrodef{C-RAN}[C-RAN]{cloud-RAN}
\acrodef{RRH}[RRH]{remote radio head}
\acrodef{BBU}[BBU]{baseband unit}
\acrodef{CS}[CS]{coordinated scheduling}
\acrodef{CB}[CB]{coordinated beamforming}
\acrodef{JT}[JT]{joint transmission}
\acrodef{NC-JT}[NC-JT]{non-coherent \ac{JT}}
\acrodef{C-JT}[C-JT]{coherent \ac{JT}}
\acrodef{DPS}[DPS]{dynamic point selection}
\acrodef{TTI}[TTI]{transmission time interval}
\acrodef{UE}[UE]{user equipment}
\acrodef{RNTP}[RNTP]{relative narrowband transmission power}
\acrodef{eRNTP}[eRNTP]{enhanced \ac{RNTP}}
\acrodef{OI}[OI]{overload indicator}
\acrodef{HII}[HII]{high interference indicator}
\acrodef{HG}[HG]{Hermite-Gaussian}
\acrodef{CQI}[CQI]{channel quality indicator}
\acrodef{PMI}[PMI]{precoding matrix indicator}
\acrodef{RI}[RI]{rank indicator}
\acrodef{HetNet}[HetNet]{heterogeneous network}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SINR}[SINR]{signal-to-interference-plus-noise ratio}
\acrodef{SC}[SC]{single-carrier}
\acrodef{SM-OFDM}[SM-OFDM]{Spatial modulation-OFDM}
\acrodef{GB}[GB]{guard band}
\acrodef{DL}[DL]{downlink}
\acrodef{UL}[UL]{uplink}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{5G}[5G]{fifth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{SISO}[SISO]{single-input single-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{LoS}[LoS]{line-of-sight}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{IoE}[IoE]{Internet of Everything}
\acrodef{SI}[SI]{self-interference}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality-of-service}
\acrodef{ITS}[ITS]{intelligent transportation system}
% \acrodef{TRxP}[TRxP]{transmission reception point}
\acrodef{HO}[HO]{handover}
\acrodef{TUBITAK}[TUBITAK]{Scientific and Technological Research Council of Turkey}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
\acrodefplural{GBR}[GBR]{guaranteed bit rate}
\acrodef{RB}[RB]{resource block}
\acrodef{PPP}[PPP]{Poisson point process}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{ISD}[ISD]{inter-site distance}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{BER}[BER]{bit error rate}
\acrodef{CSF}[CSF]{channel shortening filter}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{TDD}[TDD]{time-division duplex}
\acrodef{FDD}[FDD]{frequency-division duplex}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{MSSNR}[MSSNR]{maximum shortening signal-to-noise ratio}
\acrodef{PSD}[PSD]{power spectral density}
\acrodef{QPSK}[QPSK]{Quadrature Phase Shift Keying}
\acrodef{MMSE}[MMSE]{ minimum mean-squared error}
\acrodef{Rx}[Rx]{receiver}
\acrodef{Tx}[Tx]{transmitter}
\acrodef{TRCPR}[TRCPR]{\ac{Tx}-\ac{Rx} channel-based phase rotation}
\acrodef{TOCPR}[TOCPR]{\ac{Tx}-only channel-based phase rotation}
\acrodef{ML}[ML]{maximum likelihood}
\acrodef{SDCO}[SDCO]{spatially Distributed constellation obfuscation}
\acrodef{PDF}[PDF]{probability density function}
\acrodef{SER}[SER]{symbol error rate}
\acrodef{MISO}[MISO]{multiple-input single-output}
\acrodef{FD}[FD]{full-duplex}
\acrodef{AN}[AN]{artificial noise}
\acrodef{SC}[SC]{secrecy capacity}
\acrodef{IBFD}[IBFD]{in-band full-duplex}
\acrodef{KPI}[KPI]{key performance indicator}
\acrodef{VR}[VR]{virtual reality}
\acrodef{AR}[AR]{augmented reality}
\acrodef{6G}[6G]{sixth generation}
\acrodef{RF}[RF]{radio frequency}
\acrodef{PZ}[PZ]{protected zone}
\acrodef{SIC}[SIC]{\ac{SI} cancellation}
\acrodef{SA}[SA]{simulated annealing }
\acrodef{AI}[AI]{artificial intelligence}
\acrodef{BCD}[BCD]{block coordinate descent}
\acrodef{EE}[EE]{energy efficiency}

